Generalised unitarity for dimensionally regulated amplitudes within FDF

We review the Four-Dimensional-Formulation variant of the Four-Dimensional-Helicity scheme, by showing two applications of this regularisation scheme. The first one is the computation of one-loop helicity amplitudes, for which we present preliminary results for the analytic expressions of the one-loop Higgs plus five- gluon amplitudes. In the second part, we study the Colour-Kinematics duality for off-shell diagrams in gauge theories coupled to matter, showing in a diagrammatic way that the Jacobi relations for the kinematic numerators of off-shell diagrams, built with Feynman rules in axial gauge, reduce to definite set of violating terms due to the contributions of sub-graphs only.

==> FeynmanDiagrams/4gHD1a.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/ScalarDash}{0}
%
% Propagators
%
\FAProp(14.,10.)(6.,10.)(0.8,){/Cycles}{0}
\FAProp(14.,10.)(6.,10.)(-0.8,){/Cycles}{0}
%
% Vertices 
\FAVert(14.,10.){0}
\FAVert(6.,10.){0}
%
% Label for particles
%
\FALabel(0.,17.)[r]{$3$}
\FALabel(0.,10.)[r]{$2$}
\FALabel(0.,3.)[r]{$1$}
\FALabel(20.,15.)[l]{$4$}
\FALabel(20.,5.)[l]{$H$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHD1b.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
%
% Propagators
%
\FAProp(14.,10.)(6.,10.)(0.8,){/Cycles}{0}
\FAProp(14.,10.)(6.,10.)(-0.8,){/Cycles}{0}
%
% Vertices 
\FAVert(14.,10.){0}
\FAVert(6.,10.){0}
%
% Label for particles
%
\FALabel(0.,17.)[r]{$2$}
\FALabel(0.,10.)[r]{$1$}
\FALabel(0.,3.)[r]{$H$}
\FALabel(20.,15.)[l]{$3$}
\FALabel(20.,5.)[l]{$4$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHD2.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,10.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,18.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,12.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,8.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,2.)(14.,10.)(0.,){/Cycles}{0}
%
% Propagators
%
\FAProp(6.,10.)(14.,10.)(-0.8,){/Cycles}{0}
\FAProp(6.,10.)(14.,10.)(0.8,){/Cycles}{0}
%
% Vertices 
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
% Label for particles
%
\FALabel(0.,10.)[r]{$H$}
\FALabel(20.,18.)[l]{$1$}
\FALabel(20.,12.)[l]{$2$}
\FALabel(20.,8.)[l]{$3$}
\FALabel(20.,2.)[l]{$4$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHQa.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(20.,15.)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Propagators
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,6.5){0}
%
% Label for particles
%
\FALabel(0,17)[r]{$3$}
\FALabel(0,10)[r]{$2$}
\FALabel(0,3)[r]{$1$}
\FALabel(20,15)[l]{$4$}
\FALabel(20,5)[l]{$H$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHQb.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(20.,15.)(13.5,13.5)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Propagators
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,6.5){0}
%
% Label for particles
%
\FALabel(0,17)[r]{$4$}
\FALabel(0,10)[r]{$3$}
\FALabel(0,3)[r]{$2$}
\FALabel(20,15)[l]{$H$}
\FALabel(20,5)[l]{$1$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHQc.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.5,13.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Propagators
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Cycles}{0}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.5,13.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,6.5){0}
%
% Label for particles
%
\FALabel(0,17)[r]{$2$}
\FALabel(0,10)[r]{$1$}
\FALabel(0,3)[r]{$H$}
\FALabel(20,15)[l]{$3$}
\FALabel(20,5)[l]{$4$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHT1a.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){/ScalarDash}{0}
%
% Propagators
%
\FAProp(13.5,6.5)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(10.,12.5)(6.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(13.5,6.5){0}
\FAVert(10.,12.5){0}
\FAVert(6.5,6.5){0}
%
% Label for particles
%
\FALabel(0.,17.)[r]{$3$}
\FALabel(0.,10.)[r]{$2$}
\FALabel(0.,3.)[r]{$1$}
\FALabel(20.,15.)[l]{$4$}
\FALabel(20.,5.)[l]{$H$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHT1b.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.5,6.5)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Cycles}{0}
%
% Propagators
%
\FAProp(13.5,6.5)(10.,12.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(6.5,6.5)(0.,){/Cycles}{0}
\FAProp(10.,12.5)(6.5,6.5)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(13.5,6.5){0}
\FAVert(10.,12.5){0}
\FAVert(6.5,6.5){0}
%
% Label for particles
%
\FALabel(0.,17.)[r]{$2$}
\FALabel(0.,10.)[r]{$1$}
\FALabel(0.,3.)[r]{$H$}
\FALabel(20.,15.)[l]{$3$}
\FALabel(20.,5.)[l]{$4$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHT3a.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,12.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,8.)(0.,){/ScalarDash}{0}
%
% Propagators
%
\FAProp(14.,12.)(14.,8.)(0.,){/Cycles}{0}
\FAProp(14.,12.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(14.,8.)(6.,10.)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(14.,12.){0}
\FAVert(14.,8.){0}
\FAVert(6.,10.){0}
%
% Label for particles
%
\FALabel(0.,17.)[r]{$3$}
\FALabel(0.,10.)[r]{$2$}
\FALabel(0.,3.)[r]{$1$}
\FALabel(20.,15.)[l]{$4$}
\FALabel(20.,5.)[l]{$H$}
%
\end{feynartspicture}

==> FeynmanDiagrams/4gHT3b.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(14.,12.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,8.)(0.,){/Cycles}{0}
%
% Propagators
%
\FAProp(14.,12.)(14.,8.)(0.,){/Cycles}{0}
\FAProp(14.,12.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(14.,8.)(6.,10.)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(14.,12.){0}
\FAVert(14.,8.){0}
\FAVert(6.,10.){0}
%
% Label for particles
%
\FALabel(0.,17.)[r]{$2$}
\FALabel(0.,10.)[r]{$1$}
\FALabel(0.,3.)[r]{$H$}
\FALabel(20.,15.)[l]{$3$}
\FALabel(20.,5.)[l]{$4$}
%
\end{feynartspicture}

==> FeynmanDiagrams/6gT1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,18.)(6.,13.2)(0.,){/Cycles}{0}
\FAProp(0.,12.)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(0.,8.)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(0.,2.)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(6.,13.2)(14.,10.)(0.,){/Cycles}{0}
\FAProp(6.,13.2)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(14.,10.)(6.,8.93333)(0.,){/Cycles}{0}
%
% Vertices 
\FAVert(6.,13.2){0}
\FAVert(14.,10.){0}
\FAVert(6.,8.93333){0}
%
% Label for particles
%
%\FALabel(2.6679,15.0649)[tr]{$1$}
%\FALabel(2.88836,9.7891)[tr]{$2$}
%\FALabel(3.19982,7.66212)[t]{$3$}
%\FALabel(3.50302,5.09598)[tl]{$4$}
%\FALabel(16.6478,13.0187)[br]{$5$}
%\FALabel(17.3522,8.01869)[bl]{$6$}
%
\end{feynartspicture}

==> FeynmanDiagrams/6sQ1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,18.)(6.,13.2)(0.,){/Cycles}{0}
\FAProp(0.,12.)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(0.,8.)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(0.,2.)(6.,8.93333)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,12.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,8.)(0.,){/Cycles}{0}
%
% Propagators
\FAProp(6.,13.2)(14.,12.)(0.,){/ScalarDash}{0}
\FAProp(6.,13.2)(6.,8.93333)(0.,){/ScalarDash}{0}
\FAProp(14.,12.)(14.,8.)(0.,){/ScalarDash}{0}
\FAProp(14.,8.)(6.,8.93333)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(6.,13.2){0}
\FAVert(14.,12.){0}
\FAVert(14.,8.){0}
\FAVert(6.,8.93333){0}
%
% Label for particles
%
\FALabel(0,18)[r]{$4^+$}
\FALabel(0,12)[r]{$3^+$}
\FALabel(0,8)[r]{$2^+$}
\FALabel(0,2)[r]{$1^+$}
\FALabel(20,15)[l]{$5^+$}
\FALabel(20,5)[l]{$6^+$}
%
\end{feynartspicture}

==> FeynmanDiagrams/6sQ2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,18.)(6.,12.)(0.,){/Cycles}{0}
\FAProp(0.,12.)(6.,12.)(0.,){/Cycles}{0}
\FAProp(0.,8.)(6.,8.)(0.,){/Cycles}{0}
\FAProp(0.,2.)(6.,8.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,12.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,8.)(0.,){/Cycles}{0}
%
% Propagators
\FAProp(14.,12.)(14.,8.)(0.,){/ScalarDash}{0}
\FAProp(14.,12.)(6.,12.)(0.,){/ScalarDash}{0}
\FAProp(14.,8.)(6.,8.)(0.,){/ScalarDash}{0}
\FAProp(6.,12.)(6.,8.)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(14.,12.){0}
\FAVert(14.,8.){0}
\FAVert(6.,12.){0}
\FAVert(6.,8.){0}
%
% Label for particles
%
\FALabel(0,18)[r]{$4^+$}
\FALabel(0,12)[r]{$3^+$}
\FALabel(0,8)[r]{$2^+$}
\FALabel(0,2)[r]{$1^+$}
\FALabel(20,15)[l]{$5^+$}
\FALabel(20,5)[l]{$6^+$}
%
\end{feynartspicture}

==> FeynmanDiagrams/6sQ3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(0.,17.)(6.,12.8)(0.,){/Cycles}{0}
\FAProp(0.,10.)(6.,8.6)(0.,){/Cycles}{0}
\FAProp(0.,3.)(6.,8.6)(0.,){/Cycles}{0}
\FAProp(20.,17.)(14.,11.4)(0.,){/Cycles}{0}
\FAProp(20.,10.)(14.,11.4)(0.,){/Cycles}{0}
\FAProp(20.,3.)(14.,7.2)(0.,){/Cycles}{0}
%
% Propagators
\FAProp(6.,12.8)(6.,8.6)(0.,){/ScalarDash}{0}
\FAProp(6.,12.8)(14.,11.4)(0.,){/ScalarDash}{0}
\FAProp(14.,7.2)(6.,8.6)(0.,){/ScalarDash}{0}
\FAProp(14.,7.2)(14.,11.4)(0.,){/ScalarDash}{0}
%
% Vertices 
\FAVert(6.,12.8){0}
\FAVert(14.,7.2){0}
\FAVert(6.,8.6){0}
\FAVert(14.,11.4){0}
%
% Label for particles
%
\FALabel(0,17)[r]{$3^+$}
\FALabel(0,10)[r]{$2^+$}
\FALabel(0,3)[r]{$1^+$}
\FALabel(20,17)[l]{$4^+$}
\FALabel(20,10)[l]{$5^+$}
\FALabel(20,3)[l]{$6^+$}
%
\end{feynartspicture}

==> FeynmanDiagrams2/4g12.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_s^{\!1\!2}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g12f.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_q^{\!1\!2}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g13.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_s^{\!1\!3}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g13f.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_q^{\!1\!3}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g14.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_s^{\!1\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v
\end{feynartspicture}


==> FeynmanDiagrams2/4g23.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_s^{\!2\!3}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Cycles}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g24.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_s^{\!2\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Cycles}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g24f.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_q^{\!2\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Cycles}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g34.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_s^{\!3\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Cycles}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4g34f.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{C_q^{\!3\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Cycles}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gGen.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gGen1.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
%\FAProp(10,0)(10,0)(10,20){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
%\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
%\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
%\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
%\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
%\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
%\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
%\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gGenS.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
%\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(10,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(10,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(10,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(10,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v
%Vertices
\FAVert(10,7.87868){0}
\FAVert(10,12.1213){0}
%Prop
\FAProp(10,12.1213)(10,7.87868)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gGenS1.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
%\FAProp(10,0)(10,0)(10,20){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
%\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(10,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(10,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(10,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(10,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
%\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
%\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
%\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
%\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
%\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
%\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
%\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v
%Vertices
\FAVert(10,7.87868){0}
\FAVert(10,12.1213){0}
%Prop
\FAProp(10,12.1213)(10,7.87868)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gGenT.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
%\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(7.87868,10)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,10)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,10)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,10)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v
%Vertices
\FAVert(7.87868,10){0}
\FAVert(12.1213,10){0}
%Prop
\FAProp(7.87868,10)(12.1213,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gGenT1.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
%\FAProp(10,0)(10,0)(10,20){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
%\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(7.87868,10)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,10)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,10)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,10)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
%\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
%\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
%\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
%\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
%\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
%\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
%\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v
%Vertices
\FAVert(7.87868,10){0}
\FAVert(12.1213,10){0}
%Prop
\FAProp(7.87868,10)(12.1213,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gGenU.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
%\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(10,12.1213)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(10,7.87868)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(10,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(10,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v
%Vertices
\FAVert(10,7.87868){0}
\FAVert(10,12.1213){0}
%Prop
\FAProp(10,12.1213)(10,7.87868)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gGenU1.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
%\FAProp(10,0)(10,0)(10,20){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
%\FALabel(10,10)[c]{\large{$\mathbf{J}$}}
\FAProp(10,12.1213)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(10,7.87868)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(10,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(10,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
%\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
%\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
%\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
%\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
%\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
%\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
%\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v
%%Vertices
\FAVert(10,7.87868){0}
\FAVert(10,12.1213){0}
%%Prop
\FAProp(10,12.1213)(10,7.87868)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP1.tex <==
\unitlength=0.20bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{$\mathbf{F_4}$}
%\FAProp(7.87868,7.87868)(2.93,2.93)(0,){/Straight}{0}
\FAProp(7.87868,12.1213)(2.93,17.07)(0,){/Sine}{0}
\FAProp(12.1213,7.87868)(17.07,2.93)(0,){/Sine}{0}
\FAProp(12.1213,12.1213)(17.07,17.07)(0,){/Sine}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP1b.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{A_s^{\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Cycles}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP1bf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{A_q^{\!4}}$}}
%\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Cycles}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(7.87868,7.87868)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(7.87868,7.87868)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP1bs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(2.93,2.93)(2.93,2.93)(7,10){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(5.5,6)[c]{$F^{(4)}_s$}
%\FAProp(7.87868,7.87868)(2.93,2.93)(0,){/Straight}{0}
\FAProp(2.93,9.8)(2.93,17.07)(0,){/Straight}{0}
\FAProp(7.1213,2.93)(17.07,2.93)(0,){/Straight}{0}
\FAProp(8.5,8.5)(17.07,17.07)(0,){/Straight}{0}%largo
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
%\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
%\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP2.tex <==
\unitlength=0.20bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{$\mathbf{F_1}$}
\FAProp(7.87868,7.87868)(2.93,2.93)(0,){/Sine}{0}
%\FAProp(7.87868,12.1213)(2.93,17.07)(0,){/Straight}{0}
\FAProp(12.1213,7.87868)(17.07,2.93)(0,){/Sine}{0}
\FAProp(12.1213,12.1213)(17.07,17.07)(0,){/Sine}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP2b.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{A_s^{\!1}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP2bf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{A_q^{\!1}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
%\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(7.87868,12.1213)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(7.87868,12.1213)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP2bs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
%\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(2.93,17.07)(2.93,17.07)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(6.5,15)[c]{$F^{(1)}_s$}
\FAProp(2.93,12.87868)(2.93,2.93)(0,){/Straight}{0}
%\FAProp(7.87868,12.1213)(2.93,17.07)(0,){/Straight}{0}
\FAProp(8.5,11.5)(17.07,2.93)(0,){/Straight}{0}
\FAProp(10.1213,17.07)(17.07,17.07)(0,){/Straight}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
%\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
%\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP3.tex <==
\unitlength=0.20bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{$\mathbf{F_2}$}
\FAProp(7.87868,7.87868)(2.93,2.93)(0,){/Sine}{0}
\FAProp(7.87868,12.1213)(2.93,17.07)(0,){/Sine}{0}
\FAProp(12.1213,7.87868)(17.07,2.93)(0,){/Sine}{0}
%\FAProp(12.1213,12.1213)(17.07,17.07)(0,){/Straight}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP3b.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{B_s^{\!2}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Cycles}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP3bf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{B_q^{\!2}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{0}% Done p3
%\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Cycles}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(12.07,12.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(12.07,12.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP3bs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(17.07,17.07)(17.07,17.07)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(14,15)[c]{$\mathbf{F_2}$}
\FAProp(11.47868,11.47868)(2.93,2.93)(0,){/Straight}{0}%largo
\FAProp(9.87868,17.07)(2.93,17.07)(0,){/Straight}{0}
\FAProp(17.07,12.87868)(17.07,2.93)(0,){/Straight}{0}
%\FAProp(12.1213,12.1213)(17.07,17.07)(0,){/Straight}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
%\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
%\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP4.tex <==
\unitlength=0.20bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{$\mathbf{F_3}$}
\FAProp(7.87868,7.87868)(2.93,2.93)(0,){/Sine}{0}
\FAProp(7.87868,12.1213)(2.93,17.07)(0,){/Sine}{0}
%\FAProp(12.1213,7.87868)(17.07,2.93)(0,){/Straight}{0}
\FAProp(12.1213,12.1213)(17.07,17.07)(0,){/Sine}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gP4b.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{B_s^{\!3}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Cycles}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP4bf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\tiny{$\mathbf{B_q^{\!3}}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Straight}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Straight}{0}% Done p1
%\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Cycles}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(12.1213,7.87868)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(12.1213,7.87868)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/4gP4bs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)
\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(17.07,2.93)(17.07,2.93)(10,7){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(14,5)[c]{$\mathbf{F_3}$}
\FAProp(9.87868,2.93)(2.93,2.93)(0,){/Straight}{0}
\FAProp(11.5,8.5)(2.93,17.07)(0,){/Straight}{0}
\FAProp(17.1213,7.1213)(17.07,17.07)(0,){/Straight}{0}
% Vertices
%\FAVert(2.93,2.93){1}
%\FAVert(2.93,17.07){1}
%\FAVert(17.07,2.93){1}
%\FAVert(17.07,17.07){1}
% External particles
%\FAProp(-2,10)(-7,10)(0,){/Straight}{0}
%\FAProp(22,10)(27,10)(0,){/Straight}{0}
\end{feynartspicture}


==> FeynmanDiagrams2/4gf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\small{$\mathbf{J}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Cycles}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Cycles}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/Straight}{1}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/Straight}{-1}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}

==> FeynmanDiagrams2/4gs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(270,270)(1,1)

\FADiagram{}
%\FAVert(0.,0.){0}
%\FAVert(0.,20.){0}
%\FAVert(20.,0.){0}
%\FAVert(20.,20.){0}
\FAProp(10,7)(10,7)(10,13){/Straight}{0}
\FAProp(10,0)(10,0)(10,20){/Straight}{0}
\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAProp(10,-2)(10,-2)(10,22){/Straight}{0}
%\FAVert(10.,10.){2}
\FALabel(10,10)[c]{\small{$\mathbf{J}$}}
\FAProp(7.87868,7.87868)(4.93,4.93)(0,){/Cycles}{0}% Done p4
\FAProp(7.87868,12.1213)(4.93,15.07)(0,){/Cycles}{0}% Done p1
\FAProp(12.1213,7.87868)(15.07,4.93)(0,){/ScalarDash}{0}% Done p3
\FAProp(12.1213,12.1213)(15.07,15.07)(0,){/ScalarDash}{0}%Done p2
%"external lines"
\FAProp(4.93,15.07)(4.93,18.5)(0,){/Straight}{0}% Done p1v
\FAProp(4.93,15.07)(1.5,15.07)(0,){/Straight}{0}% Done p1h
\FAProp(15.07,15.07)(18.5,15.07)(0,){/Straight}{0}%Done p2h
\FAProp(15.07,15.07)(15.07,18.5)(0,){/Straight}{0}%Done p2v
\FAProp(15.07,4.93)(18.5,4.93)(0,){/Straight}{0}% Done p3
\FAProp(15.07,4.93)(15.07,1.5)(0,){/Straight}{0}% Done p3
\FAProp(4.93,4.93)(4.93,1.5)(0,){/Straight}{0}% Done p4h
\FAProp(4.93,4.93)(1.5,4.93)(0,){/Straight}{0}% Done p4v

\end{feynartspicture}


==> FeynmanDiagrams2/bcj.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Straight}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Straight}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/Straight}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/Straight}{0}
\FAVert(10.,10.){0}
%%\FADiagram{}
%\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{0}
%\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{0}
%% Propagator
%\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
%% Vertices
%\FAVert(10.,14.){0}
%\FAVert(10.,6.){0}
%% blob
\GOval(22.2,15.6)(7,7)(0){1.}
% labeling
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}
%\FALabel(0,15)[r]{$1$}
%\FALabel(0,5)[r]{$4$}
%\FALabel(20,15)[l]{$2$}
%\FALabel(20,5)[l]{$3$}
\FALabel(10,10)[]{\large{$\mathbf{J}$}}
\end{feynartspicture}


==> FeynmanDiagrams2/bcjf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,12.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,8.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(12.,12.)(0.,){/Straight}{1}
\FAProp(20.,5.)(12.,8.)(0.,){/Straight}{-1}
\FAVert(10.,10.){0}
%%\FADiagram{}
%\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{0}
%\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{0}
%% Propagator
%\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
%% Vertices
%\FAVert(10.,14.){0}
%\FAVert(10.,6.){0}
%% blob
\GOval(22.2,15.6)(7,7)(0){1.}
% labeling
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}
\FALabel(10,10)[]{\textbf{J}}
\end{feynartspicture}


==> FeynmanDiagrams2/bcjg.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAVert(10.,10.){0}
%%\FADiagram{}
%\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{0}
%\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{0}
%% Propagator
%\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
%% Vertices
%\FAVert(10.,14.){0}
%\FAVert(10.,6.){0}
%% blob
\GOval(22.2,15.6)(7,7)(0){1.}
% labeling
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}
\FALabel(10,10)[]{\textbf{J}}
\end{feynartspicture}


==> FeynmanDiagrams2/bcjgs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/ScalarDash}{0}
\FAVert(10.,10.){0}
%%\FADiagram{}
%\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{0}
%\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{0}
%\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{0}
%% Propagator
%\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
%% Vertices
%\FAVert(10.,14.){0}
%\FAVert(10.,6.){0}
%% blob
\GOval(22.2,15.6)(7,7)(0){1.}
% labeling
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}
\FALabel(10,10)[]{\textbf{J}}
\end{feynartspicture}


==> FeynmanDiagrams2/s.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
%\FADiagram{$n_s$}
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{0}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

%\FALabel(0,15)[r]{$1$}
%\FALabel(0,5)[r]{$4$}
%\FALabel(20,15)[l]{$2$}
%\FALabel(20,5)[l]{$3$}

\end{feynartspicture}


==> FeynmanDiagrams2/sf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{$n_1$}
%\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

\end{feynartspicture}


==> FeynmanDiagrams2/sg.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{$n_1$}
%\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/Cycles}{0}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

\end{feynartspicture}


==> FeynmanDiagrams2/sgs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{$n_1$}
%\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{0}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

\end{feynartspicture}


==> FeynmanDiagrams2/t.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)

%\FADiagram{$n_t$}
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{0}
% Propagator
\FAProp(6.,10.)(14.,10.)(0.,){/Straight}{0}
% Vertices
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

%\FALabel(0,15)[r]{$1$}
%\FALabel(0,5)[r]{$4$}
%\FALabel(20,15)[l]{$2$}
%\FALabel(20,5)[l]{$3$}

\end{feynartspicture}



==> FeynmanDiagrams2/tf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)

\FADiagram{$n_2$}
%\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
% Propagator
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
% Vertices
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}


\end{feynartspicture}



==> FeynmanDiagrams2/tg.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)

\FADiagram{$n_2$}
%\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
% Propagator
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
% Vertices
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}



\end{feynartspicture}



==> FeynmanDiagrams2/tgs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)

\FADiagram{$n_2$}
%\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/ScalarDash}{0}
% Propagator
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
% Vertices
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}



\end{feynartspicture}



==> FeynmanDiagrams2/u.tex <==
\unitlength=0.15bp%
\begin{feynartspicture}(300,200)(1,1)
%\FADiagram{$n_u$}
\FADiagram{}
\FAProp(0.,15.)(10.,6.)(0.,){/Straight}{0}
\FAProp(0.,5.)(10.,14.)(0.,){/Straight}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{0}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

%\FALabel(0,15)[r]{$1$}
%\FALabel(0,5)[r]{$4$}
%\FALabel(20,15)[l]{$2$}
%\FALabel(20,5)[l]{$3$}

\end{feynartspicture}


==> FeynmanDiagrams2/uf.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{$n_3$}
%\FADiagram{}
\FAProp(0.,15.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}

\end{feynartspicture}


==> FeynmanDiagrams2/ug.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{$n_3$}
%\FADiagram{}
\FAProp(0.,15.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/Cycles}{0}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}


\end{feynartspicture}


==> FeynmanDiagrams2/ugs.tex <==
\unitlength=0.15bp%

\begin{feynartspicture}(300,200)(1,1)
\FADiagram{$n_3$}
%\FADiagram{}
\FAProp(0.,15.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{0}
% Propagator
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
% Vertices
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}

\FALabel(0,5)[r]{$4$}
\FALabel(0,15)[r]{$1$}
\FALabel(20,15)[l]{$2$}
\FALabel(20,5)[l]{$3$}


\end{feynartspicture}


==> FeynmanRules/FF.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/Straight}{1}
\FALabel(5.5,8.93)[t]{\tiny $i$}
\FALabel(14.5,8.93)[t]{\tiny $j$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/FFG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Straight}{1}
\FALabel(5.3,8.93)[t]{\tiny $1, i$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Straight}{-1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, j$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/FFS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Straight}{1}
\FALabel(5.3,8.93)[t]{\tiny $1, i$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, B$}
\FAProp(16.,5.)(10.,10.)(0.,){/Straight}{-1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, j$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/Cycles}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, \alpha$}
\FALabel(14.5,8.93)[t]{\tiny $b, \beta$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGGG.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,12.)[]{\tiny $1,a,\alpha$}
\FAProp(10.,10.)(4.,5.)(0.,){/Cycles}{0}
\FALabel(3.0,8.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(11.,15.)[]{\tiny $2,b,\beta$}
\FAProp(10.,10.)(16.,5.)(0.,){/Cycles}{0}
\FALabel(11,5.)[]{\tiny $3,c,\gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, B$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GGS_copy.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, A$}
%\FALabel(5.5,8.93)[t]{\tiny $1, a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/GSS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1,a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, B$}
\FAProp(16.,5.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3,c, C$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/P3.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.3749)[br]{\tiny $b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,6.01315)[tr]{\tiny $c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/P4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,13.)[]{\tiny $1,a,\alpha$}
\FAProp(4.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,7.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(14.7868,13.4064)[]{\tiny $g_1$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(15.2132,8.40636)[]{\tiny $g_2$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/PRO.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,10.0)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(1.,10.0)(4.,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,10.0)(13.5,10.0)(0.,){/Straight}{-1}
\FAProp(16.,10.0)(19.0,10.0)(0.,){/GhostDash}{0}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Straight}{1}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
\FALabel(10.0,5.5)[]{\tiny $\bar \ell$}
%
\end{feynartspicture}

==> FeynmanRules/PRO.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRules/PRO.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
%\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
%\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(3.5,10.0)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(1.,10.0)(3.5,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
\FALabel(14.8,10.0)[]{\tiny $\bar \ell$}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
%\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRules/PRO.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
%\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
%\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(3.5,10.0)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(1.,10.0)(3.5,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
%\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
\FALabel(9.5,14.0)[]{\tiny $\bar \ell +p$}
\FALabel(10.0,6.0)[]{\tiny $\bar \ell$}
%
\end{feynartspicture}

==> FeynmanRules/SS.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, A$}
\FALabel(14.5,8.93)[t]{\tiny $b, B$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/SS1.tex <==
\unitlength=0.25bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a,A$}
\FALabel(14.5,8.93)[t]{\tiny $b, B$}
%\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\FAProp(10.,6.)(10.,14.)(0.,){/GhostDash}{0}
\end{feynartspicture}

==> FeynmanRules/SSGG.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,12.)[]{\tiny $1,a,\alpha$}
\FAProp(10.,10.)(4.,5.)(0.,){/Cycles}{0}
\FALabel(3.0,8.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(11.,15.)[]{\tiny $2,b,B$}
\FAProp(10.,10.)(16.,5.)(0.,){/ScalarDash}{0}
\FALabel(11,5.)[]{\tiny $3,c,C$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/gogo.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/GhostDash}{1}
\FALabel(5.5,8.93)[t]{\tiny $a$}
\FALabel(14.5,8.93)[t]{\tiny $b$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRules/gogoG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/GhostDash}{-1}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b$}
\FAProp(16.,5.)(10.,10.)(0.,){/GhostDash}{1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c$}
\FAVert(10.,10.){0}
\end{feynartspicture}
